Computing the optimal keyboard through a geometric analysis of the English language

In the context of a group project for the course COMSW4995 002 - Geometric Data Analysis, we bring our attention to the design of fast-typing keyboards. Leveraging some geometric tools in an optimization framework allowed us to propose novel keyboard layouts that offer a faster typing.

==> afaire.tex <==
plot figures
interpretations
results (plusieurs results avec plusieurs sets de paramètres)

framework de test du keyboard
optimal h1
